Fast and Simple Spectral Clustering in Theory and Practice

Spectral clustering is a popular and effective algorithm designed to find $k$ clusters in a graph $G$. In the classical spectral clustering algorithm, the vertices of $G$ are embedded into $\mathbb{R}^k$ using $k$ eigenvectors of the graph Laplacian matrix. However, computing this embedding is computationally expensive and dominates the running time of the algorithm. In this paper, we present a simple spectral clustering algorithm based on a vertex embedding with $O(\log(k))$ vectors computed by the power method. The vertex embedding is computed in nearly-linear time with respect to the size of the graph, and the algorithm provably recovers the ground truth clusters under natural assumptions on the input graph. We evaluate the new algorithm on several synthetic and real-world datasets, finding that it is significantly faster than alternative clustering algorithms, while producing results with approximately the same clustering accuracy.

==> sections/onevector.tex <==
\newcommand{\hatt}{\widehat{t}}
\newcommand{\hatu}{\widehat{u}}
\newcommand{\vmin}{v_{\mathrm{min}}}
\newcommand{\phiin}{\phi_{\mathrm{in}}}
\newcommand{\phiout}{\phi_{\mathrm{out}}}
\newcommand{\vecpsi}{\vec{\psi}}
\newcommand{\infnorm}[1]{\norm{#1}_\infty}
\newcommand{\lonenorm}[1]{\norm{#1}_1}
\newcommand{\matpi}{\matp_i}
\newcommand{\hatvecy}{\widehat{\vecy}}

\section{Graph Clustering with One Vector}
\begin{itemize}
    \item Let $\geqvew$ be a weighted undirected graph with $n$ vertices.
    % \item Let $\rho_\graphg(k) \leq \left(1 / \log(\vol(\vertexset))\right)^2$
    \item Assume $\graphg$ is $(k, \phiin, \phiout)$-clusterable
    \item Let $\sets_1, \ldots, \sets_k \subset \vertexset$ be the $k$ ground-truth sets.
    \item Let $\vmin = \min_{i \in [k]} \vol(\sets_i)$.
    \item Let $\matm = (1/2) (\identity - \adj \degm^{-1})$ be the lazy random walk matrix.
    \item Let $\vecx_0 \in \R^n$ be a random vector sampled such that $\vecx_0(u) \sim \mathrm{IW}(\deg(u))$, where $\mathrm{IW}(x)$ is the Irwin-Hall distribution with parameter $x$.
    \item For $i \in [k]$, let $t_i = \sum_{u \in \sets_i} \vecx_0(u)$. Let $\hatt_i = t_i / \vol(\sets_i)$.
\end{itemize}

\todo{add definition of in/out clusterable}

\todo{introduce the Irwin-Hall distribution}

We will make use of the Berry-Esseen theorem, which guarantees that the sum of independent random variables is well approximated by the normal distribution.
\begin{theorem}[Berry-Esseen.]
Let $X_1, X_2, \ldots, X_n$ be independent random variables with $\E\left[X_j\right] = 0$, $\E\left[X_j^2\right] = \sigma_j^2 > 0$, and $\E\left[\abs{X_j}^3\right] = \rho_j < \infty$.
Let
\[
    S = \frac{\sum_{j = 1}^n X_j}{\sqrt{\sum_{j = 1}^n \sigma_j^2}},
\]
let $F: \R \rightarrow [0, 1]$ be the CDF of $S$, and let $\Phi: \R \rightarrow [0, 1]$ be the CDF of the standard normal distribution.
Then,
\[
    \sup_{x \in \R} \abs{F(x) - \Phi(x)} \leq \sqrt{\sum_{j=1}^n \sigma_j^2} \cdot \max_{1 \leq j \leq n} \left(\frac{\rho_j}{\sigma_j^2}\right).
\]
\end{theorem}

\begin{lemma}
With probability at least $1 - (2 k^2 / \sqrt{\vmin})$, it holds that
\[
    \abs{\hatt_i - \hatt_j} \geq \frac{1}{\vmin},
\]
for all $i, j \in [k]$ with $i \neq j$.
\end{lemma}

\begin{proof}
Since $t_i$ is a sum of random variables distributed according to the Irwin-Hall distribution, $t_i$ can be viewed as a sum of random variables distributed according to the uniform distribution:
\[
    t_i = \sum_{k=1}^{\vol(\sets_i)} u_{i, k},
\]
where $u_{i, k} \sim U(0, 1)$.
We can also rewrite $\hatt_i$ as
\begin{align*}
    \hatt_i & = \sum_{k=1}^{\vol(\sets_i)} \frac{u_{i, k}}{\vol(\sets_i)} \\
    & = \frac{1}{2} + \sum_{k = 1}^{\vol(\sets_i)} \hatu_{i, k},
\end{align*}
where $\hatu_{i, k} = (u_{i, k} - (1 / 2)) / \vol(\sets_i)$, which implies that
\[
\hatu_{i, k} \sim U\left(-\frac{1}{2 \vol(\sets_i)}, \frac{1}{2 \vol(\sets_i)}\right).
\]
By similarly defining $\hatu_{j, k}$ and by the symmetry of the distribution of $\hatu_{j, k}$,
we have that
\begin{align*}
    \hatt_i - \hatt_j = \sum_{k = 1}^{\vol(S_i)} \hatu_{i, k} + \sum_{k = 1}^{\vol(\sets_j)} \hatu_{j, k}.
\end{align*}
As such, $\hatt_i - \hatt_j$ is a sum of independent random variables.
In order to apply the Berry-Esseen theorem, we will use the following facts, which are easily derived from the properties of the uniform distribution.
\begin{itemize}
    \item $\E\left[\hatu_{i, k}\right] = 0$.
    \item $\sigma_{i, k}^2 \triangleq \E\left[\hatu_{i, k}^2\right] = \frac{1}{12 \vol(\sets_i)^2}$.
    \item $\rho_{i, k} \triangleq \E\left[\abs{\hatu_{i, k}}^3\right] = \frac{1}{36 \vol(\sets_i)^3}$.
\end{itemize}
Then, let
\[
    s \triangleq \sqrt{\sum_{k = 1}^{\vol(\sets_i)} \sigma_{i, k}^2 + \sum_{k = 1}^{\vol(\sets_j)} \sigma_{j, k}^2} = \sqrt{\frac{1}{12 \vol(\sets_i)} + \frac{1}{12 \vol(\sets_j)}}
    \leq \frac{1}{\sqrt{6 v}},
\]
where $v = \min_{1 \leq i \leq k} \vol(\sets_i)$.
Let
\[
    S = \frac{\hatt_i - \hatt_j}{s}.
\]
Then, we can apply the Berry-Esseen theorem which gives that
\[
    \sum_{x \in \R} \abs{F(x) - \Phi(x)} \leq \frac{1}{3 \sqrt{6} v},
\]
where $F$ is the CDF of $S$.
We have that
\begin{align*}
    \P\left[ \abs{\hatt_i - \hatt_j} > 1 / v \right]
    & = 2 \cdot \P\left[ \hatt_i - \hatt_j < - 1 / v \right] \\
    & = 2 \cdot \P\left[ S < - 1 / (s v) \right] \\
    & \geq 2 \left( \Phi(-1 / (sv)) - \frac{1}{3 \sqrt{6} v} \right) \\
    & \geq 2 \left( \frac{1}{2} - \frac{1}{\sqrt{2 \pi} s v} - \frac{1}{3 \sqrt{6} v}\right) \\
    & \geq 2 \left( \frac{1}{2} - \sqrt{\frac{3}{\pi v}} - \frac{1}{3 \sqrt{6} v}\right) \\
    & \geq 1 - \frac{2}{\sqrt{v}}.
\end{align*}
Then, the lemma follows by the union bound.
\end{proof}

\subsection{Close to random walk on cluster}
\begin{itemize}
    \item Let $\vecx \in \R^n_+$ with $\infnorm{\degm^{-1}\vecx} \leq 1$
    \item For $\sets_i$, let $\degm_i$ be the diagonal degree matrix of the induced graph on $\sets_i$. \todo{define this formally}
    \item Let $\matm_i = \frac{1}{2} (\matpi + \adj_i \degm_i^{-1})$ be the random walk matrix on the graph induced by $\sets_i$, with $\adj_i = \matpi \adj \matpi$.
    \item \todo{define $\degm_i^{-1}$. Notice that $\degm_i = \degm_i \matpi$ and $\degm_i^{-1} = \degm_i^{-1} \matpi$.}
\end{itemize}

We will use the following result shown by Spielman and Teng~\cite{spielmanLocalClusteringAlgorithm2013}.

\begin{lemma}[\cite{spielmanLocalClusteringAlgorithm2013}, Proposition 2.2] \label{lem:monotinicity}
    For all non-negative vectors $\vecp$,
    \[
        \norm{\degm^{-1} \matm \vecp}_\infty \leq \norm{\degm^{-1} \vecp}_\infty.
    \]
\end{lemma}

\begin{lemma}
    For any $\vecx \in \R^n_+$ with $\infnorm{\degm^{-1} \vecx} \leq 1$,
    \[
        \norm{\matp_i \matm \vecx - \matm_i \matp_i \vecx}_1 \leq \weight(\sets_i, \setcomplement{\sets_i}).
    \]
\end{lemma}

\begin{proof}
    We have
    \begin{align*}
        \matpi \matm \vecx
        & = \matpi \matm \matpi \vecx + \matpi \matm \left(\identity - \matpi\right) \vecx \\
        & = \frac{1}{2} \matpi \vecx + \frac{1}{2} \adj_i \degm^{-1} \vecx + \matpi \matm \left(\identity - \matpi\right) \vecx \\
        % & = \frac{1}{2} \matpi \vecx + \frac{1}{2} \adj_i \degm_i^{-1} \left(\degm_i \degm^{-1}\right) \vecx + \matpi \matm \left(\identity - \matpi\right) \vecx \\
        & = \frac{1}{2} \matpi \vecx + \frac{1}{2} \adj_i \degm_i^{-1} \vecx - \frac{1}{2} \adj_i \degm_i^{-1} \left(\identity - \degm_i \degm^{-1}\right) \vecx + \matpi \matm \left(\identity - \matpi\right) \vecx \\
        & = \matm_i \matpi \vecx - \frac{1}{2} \adj_i \degm_i^{-1} \left(\identity - \degm_i \degm^{-1}\right) \vecx + \matpi \matm \left(\identity - \matpi\right) \vecx.
    \end{align*}
    Then, we have
    \begin{align*}
        \lonenorm{\matpi \matm \vecx - \matm_i \matpi \vecx}
        & \leq \frac{1}{2} \lonenorm{\adj_i \degm_i^{-1} \left(\identity - \degm_i \degm^{-1}\right)\vecx} + \frac{1}{2} \lonenorm{\matpi \adj \degm^{-1} \left(\identity - \matpi\right) \vecx} \\
        & = \frac{1}{2} \lonenorm{\matpi \left(\identity - \degm_i \degm^{-1}\right)\vecx} + \frac{1}{2} \lonenorm{\matpi \adj \left(\identity - \matpi\right) \degm^{-1} \vecx} \\
        & = \frac{1}{2} \lonenorm{\left(\degm - \degm_i\right) \matpi \degm^{-1} \vecx} + \frac{1}{2} \weight(\sets_i, \setcomplement{\sets_i}) \infnorm{\degm^{-1} \vecx} \\
        & \leq \frac{1}{2} \weight(\sets_i, \setcomplement{\sets_i}) \infnorm{\degm^{-1} \vecx} + \frac{1}{2} \weight(\sets_i, \setcomplement{\sets_i}) \\
        & \leq \weight(\sets_i, \setcomplement{\sets_i}),
    \end{align*}
    which completes the proof.
\end{proof}

\begin{lemma}
    For any $\vecx \in \R^n_+$,
    \[
    \norm{\matp_i \matm \vecx - \matp_i \matm \matp_i \vecx}_1 \leq \weight(\sets_i, \setcomplement{\sets_i}) \cdot \infnorm{\degm^{-1} \vecx}.
    \]
\end{lemma}

\begin{proof}
    We have 
    \begin{align*}
        \matp_i \matm \vecx - \matpi \matm \matpi \vecx & = \matpi \matm \left(\identity - \matpi\right) \vecx \\
        & = \frac{1}{2} \matpi \adj \degm^{-1} \left(\identity - \matpi\right) \vecx \\
        & = \frac{1}{2} \matpi \adj \left(\identity - \matpi\right) \degm^{-1} \vecx,
    \end{align*}
    where we use the fact that $\matpi$ is a diagonal projection matrix.
    Then,
    \begin{align*}
        \norm{\matpi \matm \vecx - \matpi \matm \matpi \vecx}_1
        & \leq \frac{1}{2} \weight(\setcomplement{\sets_i}, \sets_i) \infnorm{\degm^{-1} \vecx},
    \end{align*}
    which completes the proof of the lemma.
\end{proof}

\begin{lemma}
    For any $\vecx \in \R^n$ with $\infnorm{\degm^{-1} \vecx} \leq 1$, and any integer $t \geq 0$,
    \[
        \norm{\matp_i \matm^t \vecx - \matm_i^t \matp_i \vecx}_1 \leq
        2 \cdot t \cdot \weight(\sets_i, \setcomplement{\sets_i}).
    \]
\end{lemma}

\begin{proof}
    The proof is by induction on $t$. The base case $t = 0$ follows trivially.
    For the inductive step, we assume that the claim holds for some $t$ and establish the claim for $t + 1$.
    Let $\vecy = \matpi \matm^t \vecx$ and $\hatvecy = \matm_i^t \matpi \vecx$.
    Then, we have
    \begin{align*}
        \lonenorm{\matpi \matm^{t+1} \vecx - \matm_i^{t+1} \matpi \vecx}
        & = \lonenorm{\matpi \matm \matm^t \vecx - \matm_i \matm_i^t \matpi \vecx} \\
        & \leq \lonenorm{\matpi \matm \matm^t \vecx - \matpi \matm \left(\matpi \matm^t \vecx\right)} + \lonenorm{\matpi \matm \left(\matpi \matm^t \vecx\right) - \matm_i \left(\matm_i^t \matpi \vecx\right)} \\
        & \leq \frac{1}{2} \weight(\sets_i, \setcomplement{\sets_i}) + \lonenorm{\matpi \matm (\hatvecy + \vecy - \hatvecy) - \matm_i \hatvecy} \\
        & \leq \frac{1}{2} \weight(\sets_i, \setcomplement{\sets_i}) + \lonenorm{\matpi \matm \hatvecy - \matm_i \matpi \hatvecy} + \lonenorm{\matpi \matm (\vecy - \hatvecy)} \\
        & \leq \frac{1}{2} \weight(\sets_i, \setcomplement{\sets_i}) + \weight(\sets_i, \setcomplement{\sets_i}) + \lonenorm{\vecy - \hatvecy} \\
        & \leq 2 \weight(\sets_i, \setcomplement{\sets_i}) + 2 t \weight(\sets_i, \setcomplement{\sets_i}),
    \end{align*}
    which completes the proof of the inductive step.
\end{proof}

\subsection{Putting it all together}
We will use the following lemma for the mixing time of a random walk. The following is a standard result connecting the mixing time of a
random walk on a graph with the conductance of the graph~\cite{jerrum1988conductance}.

\begin{lemma} \label{lem:mixing}
    Given any graph $\geqvew$ with conductance $\phi_G$, and a positive vector $\vecx_0 \in \R^n$.
    Let $t = \bigtheta{\phi_G^{-2} \log(\vol(\vertexset)) \log (1 / \epsilon)}$. Then,
    \[
        \lonenorm{\matm^t \vecx_0 - \vec{\pi}} \leq \epsilon,
    \]
    where $\matm$ is the lazy random walk matrix on $\graphg$ and $\vec{\pi}$ is the stationary distribution given by 
    \[
        \vec{\pi}(u) = \frac{\deg(u)}{\vol(\vertexset)} \cdot \norm{\vecx_0}_1
    \]
    for every vertex $u \in \vertexset$.
\end{lemma}


Now, let $\vecf = \degm^{-1} \matm^t \vecx_0$ be the vector computed by applying the power method to $\vecx_0$ for $t = \bigtheta{\phiout / \phiin}$ iterations, and normalising by degrees.

\begin{lemma}
    If $\phiin / \phiout = \bigomega{\log(\vol(\vertexset))^2}$, then the following holds.
    For all $i \in [k]$ and any $u \in \sets_i$,
    \[
        \left(1 - \epsilon \right) \hatt_i \leq \vecf(u) \leq \left(1 + \epsilon \right) \hatt_i,
    \]
    where $\epsilon = 1 / \vol(\vertexset)$.
\end{lemma}

\begin{proof}
    % Let $\matp_{i}$ be the projection matrix onto the vertices in $\sets_i$. That is $\matp_i$ is diagonal with entries
    % \[
    %     \matp_{i}(u, u) = \twopartdefow{1}{u \in \sets_i}{0}.
    % \]
    % Let $\vecpsi_i = \matp_i \vecx_0$ be the initial distribution of probability mass on vertices in $\sets_i$.
    % Then, we have
    % \[
    %     \norm{\degm^{-1} \vecpsi_i}_\infty \leq 1
    % \]
    % since each $\vecpsi_i(u)$ is chosen according to the Irwin-Hall distribution with parameter $\deg(u)$.
    % Then, for \emph{any} positive vector $\vecx$ with $\infnorm{\degm^{-1} \vecx} \leq 1$,
    % \[
    %     \infnorm{\degm^{-1} (\matp_i \matm) \vecx} = \infnorm{\matp_i \degm^{-1} \matm \vecx} \leq \infnorm{\degm^{-1} \matm \vecx} \leq \infnorm{\degm^{-1} \vecx} \leq 1,
    % \]
    % where the second last inequality follows by Lemma~\ref{lem:monotinicity}.
    
    Consider some arbitrary cluster $\sets_i$ and let $\vec{\pi}_i$ be defined such that
    \[
        \vec{\pi}_i(u) = \twopartdefow{\frac{\deg(u)}{\vol(\sets_i)} \cdot t_i}{u \in \sets_i}{0}.
    \]
    Then, we have by Lemma~\ref{lem:mixing} that
    \begin{align*}
        \lonenorm{\matm_i^t \matpi \vecx_0 - \vec{\pi}_i} \leq 
    \end{align*}
\end{proof}

